Bohemian Upper Hessenberg Matrices

We look at Bohemian matrices, specifically those with entries from $\{-1, 0, {+1}\}$. More, we specialize the matrices to be upper Hessenberg, with subdiagonal entries $\pm1$. Many properties remain after these specializations, some of which surprised us. We find two recursive formulae for the characteristic polynomials of upper Hessenberg matrices. Focusing on only those matrices whose characteristic polynomials have maximal height allows us to explicitly identify these polynomials and give a lower bound on their height. This bound is exponential in the order of the matrix. We count stable matrices, normal matrices, and neutral matrices, and tabulate the results of our experiments. We prove a theorem about the only possible kinds of normal matrices amongst a specific family of Bohemian upper Hessenberg matrices.

==> MaxHeightCharPolys.tex <==
In this section we restrict our analysis to upper Hessenberg Toeplitz matrices with $-1$ on the subdiagonal and all other entries equal to $1$ (i.e. $t_k = 1$ for $1 \le k \le n$, and $s = -1$). We denote a dimension $n$ matrix of this form by $\widetilde{\mathbf{M}}_n$.
$\widetilde{\mathbf{M}}_n$ is of maximal height by Proposition~\ref{prop:maxheight_UHT2}.

\begin{proposition}
    The characteristic polynomial of $\widetilde{\mathbf{M}}_n$ is of the form
    \begin{align}
        P_n &= z^n + p_{n,n-1}z^{n-1} + \cdots + p_{n,0}\\
        &= z^n - q_{n,n-1}z^{n-1} + \cdots + (-1)^n q_{n,0}
    \end{align}
    where $q_{n,j} = (-1)^{n-j} p_{n,j}$ is positive for all $n$ and $j$.
\end{proposition}
\begin{proof}
    When $t_k = 1$ for $1 \le k \le n$, and $s = -1$, Proposition~\ref{prop:charpolyrec2_UHT} can be written in terms of $q_{n,j}$ as
    \begin{subequations}
    \label{eqn:max_height_char_poly_rec}
    \begin{align}
        q_{n,n} &= 1,\\
        q_{n,j} &= q_{n-1,j-1} + \sum_{k=1}^{n-j} q_{n-k,j}\quad\text{for}\quad 1 \le j \le n-1, \label{eqn:max_height_char_poly_rec_b}\\
        q_{n,0} &= \sum_{k=1}^n q_{n-k,0},
 \,\text{and} \label{eqn:max_height_char_poly_rec_c}\\
        q_{0,0} &= 1 \label{eqn:max_height_char_poly_rec_d}\>.
    \end{align}
    \end{subequations}
    Since $q_{0,0}$ is positive, and all coefficients in the above equations are positive, $q_{n,j}$ must be positive for all $n$ and $j$.
\end{proof}

\begin{proposition}
    \label{prop:genfun}
    The generating function of the sequence $(q_{i,i}, q_{i+1,i}, \ldots)$ for all $i \ge 0$ is
    \begin{equation}
        G_{i}(x) = \bigg (\frac{1-x}{1-2x} \bigg)^{i+1} \>.
    \end{equation}
\end{proposition}
\begin{proof}
    First we will prove the $i=0$ case. Let 
    \begin{equation}
        G_0(x) = \sum_{\ell=0}^{\infty} q_{\ell,0} x^\ell \>.
    \end{equation}
    Then,
    \begin{equation}
        (1-2x) = q_{0,0} + \sum_{\ell=1}^{\infty} (q_{\ell,0} - 2q_{\ell-1,0}) x^\ell \>.
    \end{equation}
    From equation~\eqref{eqn:max_height_char_poly_rec_c},
    \begin{align}
        (1-2x) G_0(x) &= q_{0,0} + (q_{1,0} - 2q_{0,0}) x + \sum_{\ell=2}^{\infty} (q_{\ell,0} - 2q_{\ell-1,0})x^\ell\\
        &= q_{0,0} + (q_{1,0} - 2q_{0,0}) x + \sum_{\ell=2}^{\infty} \bigg ( \sum_{k=1}^{\ell} q_{\ell-k,0} - 2 \sum_{k=1}^{\ell-1} q_{\ell-1-k,0} \bigg ) x^{\ell} \\
        &= q_{0,0} + (q_{1,0} - 2q_{0,0}) x + \sum_{\ell=2}^{\infty} \bigg ( \sum_{k=1}^{\ell} q_{\ell-k,0} - 2 \sum_{k=2}^{\ell} q_{\ell-k,0} \bigg ) x^{\ell}\\
        &= q_{0,0} + (q_{1,0} - 2q_{0,0}) x + \sum_{\ell=2}^{\infty} \bigg ( q_{\ell-1,0} - \sum_{k=2}^{\ell} q_{\ell-k,0} \bigg ) x^{\ell} \>.
    \end{align}
    Since $q_{0,0} = q_{1,0} = 1$,
    \begin{align}
        (1-2x) G_0(x) &= 1 - x + \sum_{\ell = 2}^{\infty} \bigg( q_{\ell-1,0} - \sum_{k=1} ^{\ell-1} q_{\ell-1-k,0} \bigg)x^{\ell} \\
        &= 1-x \>.
    \end{align}
    Therefore
    \begin{equation}
        G_0(x) = \frac{1-x}{1-2x} \>.
    \end{equation}
    
    Next we prove the general case for $i > 0$. Assume inductively that
    \begin{equation}
        G_i(x) = \bigg ( \frac{1-x}{1-2x} \bigg )^{i+1} = \sum_{\ell=0}^{\infty} q_{i+\ell,i} x^\ell \>.
    \end{equation}
    Then,
    \begin{align}
        G_{i+1}(x) &= \bigg ( \frac{1-x}{1-2x} \bigg )^{i+2}\\
        &= \bigg ( \frac{1-x}{1-2x} \bigg )^{i+1} \bigg ( \frac{1-x}{1-2x} \bigg )\\
        (1-2x)G_{i+1}(x) &= (1-x) \bigg ( \frac{1-x}{1-2x} \bigg )^{i+1}\\
        &= (1-x) \sum_{\ell=0}^{\infty} q_{i+\ell,i} x^{\ell} \\
        &= \sum_{\ell=0}^{\infty} q_{i+\ell,i}x^{\ell} - \sum_{\ell=0}^{\infty} q_{i+\ell,i} x^{\ell+1}\\
        &= \sum_{\ell=0}^{\infty} q_{i+\ell,i} x^{\ell} - \sum_{\ell=1}^{\infty} q_{i+\ell-1,i} x^{\ell} \\
        &= q_{i,i} + \sum_{\ell=1}^{\infty} (q_{i+\ell,i} - q_{i+\ell-1,i}) x^{\ell}\>.
    \end{align}
    Rewriting equation~\eqref{eqn:max_height_char_poly_rec_b} as
    \begin{equation}
        q_{n,j} = q_{n+1,j+1} - \sum_{k=1}^{n-j} q_{n+1-k,j+1},
    \end{equation}
    we find
    \begin{align}
    (1-2x)G_{i+1}(x) &= q_{i,i} + \sum_{\ell=1}^{\infty} \Bigg [ \bigg ( q_{i+\ell+1,i+1} - \sum_{k=1}^{\ell} q_{i+\ell+1-k,i+1} \bigg ) - \bigg ( q_{i+\ell,i+1} - \sum_{k=1}^{\ell-1} q_{i+\ell-k,i+1} \bigg ) \Bigg] x^{\ell}\\
    &= q_{i,i} + \sum_{\ell=1}^{\infty} \bigg ( q_{i+\ell+1,i+1} - q_{i+\ell,i+1} - \sum_{k=0}^{\ell-1} q_{i+\ell-k,i+1} + \sum_{k=1}^{\ell-1} q_{i+\ell-k,i+q} \bigg ) x^{\ell}\\
    &= q_{i,i} + \sum_{\ell=1}^{\infty} \bigg ( q_{i+\ell+1,i+1} - q_{i+\ell,i+1} - q_{i+\ell,i+1} \bigg ) x^{\ell}\\
    &= q_{i,i} + \sum_{\ell=1}^{\infty} (q_{i+\ell+1,i+1} - 2q_{i+\ell,i+1}) x^{\ell}\\
    &= q_{i+1,i+1} + \sum_{\ell=1}^{\infty} (q_{i+\ell+1,i+1} - 2 q_{i+\ell,i+1}) x^{\ell}\\
    &= \sum_{\ell=0}^{\infty} q_{i+\ell+1,i+1} x^{\ell} - 2x \sum_{\ell = 0}^{\infty} q_{i+\ell+1,i+1}x^{\ell}\\
    &= (1-2x) \sum_{\ell=0}^{\ell} q_{i+\ell+1,i+1} x^{\ell}\>.
    \end{align}
    Therefore,
    \begin{equation}
        G_{i+1}(x) = \sum_{\ell=0}^{\infty} q_{i+\ell+1,i+1} x^{\ell} = \bigg ( \frac{1-x}{1-2x} \bigg )^{i+2}\>.
    \end{equation}
\end{proof}

\begin{proposition}
    The coefficients $q_{n,k}$ are given by the OEIS sequence \href{http://oeis.org/A105306}{A105306} for the ``number of directed column-convex polynomials of area $n$, having the top of the right-most column at height $k$.'' We have $q_{n,k} = T_{n+1,k+1}$ where
    \begin{equation}
        T_{n,k} = 
        \begin{cases}
            \displaystyle\sum_{j=0}^{n-k-1} \binom{k+j}{k-1} \binom{n-k-1}{j} & \text{if } k < n\\
            \hfil 1 & \text{if } k = n
        \end{cases}
    \end{equation}
    Maple simplifies this to
    \begin{equation}
      T_{n,k} =
      \begin{cases}
          kF \!
          \left(
              \begin{array}{c|c}
                  k+1, k+1-n & \multirow{2}{*}{$-1$} \\
                  2 &
              \end{array}
          \right) & \text{if } n \ne k\\
          \hfil 1 & \text{if } n = k
        \end{cases}
    \end{equation}
    where $F(\cdot)$ is the hypergeometric function defined as
    \begin{equation}
        F \!
          \left(
              \begin{array}{c|c}
                  a, b & \multirow{2}{*}{$z$} \\
                  c &
              \end{array}
          \right)
          =
          \sum_{n=0}^{\infty} \frac{(a)_n (b)_n}{(c)_n} \frac{z^n}{n!}
    \end{equation}
    where $(q)_n = q(q+1)\cdots(q+n-1)$ is the Pochhammer symbol.
\end{proposition}
\begin{proof}
    We will show that
    \begin{equation}
        q_{i+n,i} = T_{n+i+1,i+1} =
        \begin{cases}
            \displaystyle \sum_{j=0}^{n-1} {i+j+1 \choose i} {n-1 \choose j} & \text{if } n > 0\\
            \hfil 1 & \text{if } n = 0 \>.
        \end{cases}
    \end{equation}

    By Proposition~\ref{prop:genfun}
    \begin{equation}
        q_{i+n,i} = \frac{1}{n!} \frac{\mathrm{d}^n}{\mathrm{d}x^n} G_i(x) \Bigr|_{x=0}
    \end{equation}
    where
    \begin{equation}
        G_i(x) = \bigg ( \frac{1-x}{1-2x} \bigg )^{i+1} = f_i(g_i(x))
    \end{equation}
    with
    \begin{align}
        f_i(x) &= x^{i+1}, \text{ and}\\
        g_i(x) &= \frac{1-x}{1-2x} = \frac{1}{1-2x} - \frac{x}{1-2x}\>.
    \end{align}
    Differentiating $f_i(x)$ and $g_i(x)$ with respect to $x$,
    \begin{align}
        \frac{\mathrm{d}^n}{\mathrm{d}x^n} f_i(x) &=
        \begin{cases}
            (i+1)(i)\cdots(i-n+2) x^{i+1-n} &\text{for}\quad n \le i+1\\
            \hfil 0 &\text{for}\quad n > i+1
        \end{cases}\\
        &= {i+1 \choose n} n! x^{i+1-n}
    \end{align}
    and
    \begin{align}
        \frac{\mathrm{d}^n}{\mathrm{d}x^n} g_i(x) &= \frac{\mathrm{d}^n}{\mathrm{d}x^n} \frac{1}{1-2x} + \frac{\mathrm{d}^n}{\mathrm{d}x^n} \frac{x}{1-2x}\\
        &= \frac{2^n n!}{(1-2x)^{n+1}} + \frac{2^{n-1} n!}{(1-2x)^n} + \frac{2^n n! \,x}{(1-2x)^{n+1}}\\
        &= \frac{2^n n! (1-x)}{(1-2x)^{n+1}} - \frac{2^{n-1}n!}{(1-2x)^n}
    \end{align}
    with
    \begin{equation}
    \frac{\mathrm{d}^n}{\mathrm{d}x^n} g_i(x) \Bigr|_{x=0} =
    \begin{cases}
        n!\,2^{n-1} &\text{for}\quad n > 0\\
        1 &\text{for}\quad n = 0 \>.
    \end{cases}
    \end{equation}
    
    When $n=0$,
    \begin{equation}
        q_{i+n,i} = q_{i,i} = G_i(0) = 1 \>.
    \end{equation}
    For $n > 0$, by Fa\`a di Bruno's formula we have
    \begin{align}
        \frac{\mathrm{d}^n}{\mathrm{d}x^n} G_i(x) &= \frac{\mathrm{d}^n}{\mathrm{d}x^n} f_i(g_i(x)) \\
        &= \sum_{k=1}^n f_i^{(k)}\big(g_i(x)\big) B_{n,k} (g_i'(x), g_i''(x), \ldots, g_i^{(n-k+1)}(x))
    \end{align}
    and therefore
    \begin{align}
        \frac{\mathrm{d}^n}{\mathrm{d}x^n} G_i(x) \Bigr|_{x=0} &= \sum_{k=1}^n f_i^{(k)} \big ( g_i(0) \big) B_{n,k} (g_i'(0), g_i''(0), \ldots, g_i^{(n-k+1)}(0))\\
        &= \sum_{k=1}^n f_i^{(k)}(1) B_{n,k}(1, 4, 24, \ldots, (n-k+1)! 2^{n-k}) \>.
    \end{align}
    
    By Theorem 6 of~\cite{abbas2005new},
    \begin{align}
         B_{n,k}(1, 4, 24, \ldots, (n-k+1)! 2^{n-k}) &= B_{n,k}(p_0(1), p_1(2), \ldots, p_{n-k}(n-k+1)) \\
         &= {n-1 \choose k-1} \frac{n!}{k!} 2^{n-k}
    \end{align}
    because
    \begin{equation}
        p_n(x) = \frac{x!}{(x-n)!} 2^n
    \end{equation}
    satisfies
    \begin{equation}
        p_n(x+y) = \sum_{k=0}^n {n \choose k} p_k(y) p_{n-k}(x) \>.
    \end{equation}
    
    Returning to the proof,
    \begin{align}
        q_{i+n,i} &= \frac{1}{n!} \frac{\mathrm{d}^n}{\mathrm{d}x^n} G_i(x)\Bigr|_{x=0} \\
        &= \frac{1}{n!} \sum_{k=1}^n {i+1 \choose k} {n-1 \choose k-1} k! \frac{n!}{k!} 2^{n-k} \\
        &= \sum_{k=1}^n {i+1 \choose k} {n-1 \choose k-1} 2^{n-k} \\
        &= \sum_{k=0}^{n-1} {i+1 \choose k+1} {n-1 \choose k} 2^{n-k-1} \\
        &= \sum_{k=0}^{n-1} {i+1 \choose k+1} {n-1 \choose k} \sum_{j = 0}^{n-k-1} {n-k-1 \choose j}\\
        &= \sum_{k=0}^{n-1} \sum_{j=0}^{n-k-1} {n-1 \choose k} {i+1 \choose k+1} {n-k-1 \choose j}\\
        &= \sum_{j = 0}^{n-1} \sum_{k = 0}^{n - j - 1} {n-1 \choose k} {i+1 \choose k+1} {n-k-1 \choose j}\\
        &= \sum_{j = 0}^{n-1} \sum_{k=0}^{j} {n-1 \choose k} {i+1 \choose k+1} {n-k-1 \choose n-j - 1}\\
        &= \sum_{j = 0}^{n-1} \sum_{k=0}^{j} {n-1 \choose n-j - 1} {j \choose k} {i+1 \choose k+1}\\
        &= \sum_{j = 0}^{n-1} {n-1 \choose j} \sum_{k=0}^{j} {j \choose k} {i+1 \choose k+1} \\
        &= \sum_{j = 0}^{n-1} {n-1 \choose j} {i+j+1 \choose j + 1} \\
        &= \sum_{j = 0}^{n-1} {n-1 \choose j} {i+j+1 \choose i}
    \end{align}
    %%% OLD
    % %     
    % % \end{align}
    
    % Proof that
    % \begin{equation}
    %     B_{n,k}(1, 4, 24, \ldots, (n-k+1)! 2^{n-k}) = {n-1 \choose k-1} \frac{n!}{k!} 2^{n-k} \>.
    % \end{equation}
    % Let
    % \begin{equation}
    % \   p_n(x) = \frac{x!}{(x-n)!} 2^n \>.
    % \end{equation}
    % By Theorem 6 of~\cite{abbas2005new}, if $p_n(x)$ satisfies
    % \begin{equation}
    %     p_n(x+y) = \sum_{k=0}^n {n \choose k} p_k(y) p_{n-k}(x),
    % \end{equation}
    % then
    % \begin{equation}
    %     B_{n,k} (p_0(1), p_1(2), \ldots) = {n-1 \choose k-1} p_{n-k}(n) \>.
    % \end{equation}
    % $p_{n-1}(n)$ satisfies
    % \begin{equation}
    %     p_{n-1}(n) = \frac{n!}{(n-(n-1))!} 2^{n-1} = n! 2^{n-1} = g_i^{(n)}(0) \>.
    % \end{equation}
    % \begin{align}
    % \sum_{k=0}^n {n \choose k} p_k(y) p_{n-k}(x) &= \sum_{k=0}^n {n \choose k} \frac{y!}{(y-k)!} 2^k \frac{x!}{(x-(n-k))!} 2^{n-k} \\
    % &= \sum_{k=0}^n {n \choose k} \frac{y!}{(y-k)!} \frac{x!}{(x-n-k)!} 2^n \\
    % &= 2^n \sum_{k=0}^n {n \choose k} {y \choose k} {x \choose n-k} k! (n-k)! \\
    % &= 2^n \sum_{k=0}^n n! {y \choose k} {x \choose n-k}\\
    % &= n! 2^n {x+y \choose n}\\
    % &= \frac{(x+y)!}{(x+y-n)!} 2^n = p_n(x+y) \>.
    % \end{align}
    
    % Returning to the original proof,
    % \begin{align}
    %     q_{i+n,i} &= \frac{\frac{d^n}{dx^n} G_i(0)}{n!} \\
    %     &= \frac{1}{n!} \sum_{k=1}^n {i+1 \choose k} {n-1 \choose k-1} n! 2^{n-k}\\
    %     &= \sum_{k=1}^n {i+1 \choose k} {n-1 \choose k-1} 2^{n-k} \\
    %     &= \sum_{k=0}^{n-1} {i+1 \choose k+1} {n-1 \choose k} 2^{n-k-1} \\
    %     &= \sum_{k=0}^{n-1} {i+1 \choose k+1} {n-1 \choose k} \sum_{\ell = 0}^{n-k-1} {n-k-1 \choose \ell}\\
    %     &= \sum_{k=0}^{n-1} \sum_{\ell=0}^{n-k-1} {n-1 \choose k} {i+1 \choose k+1} {n-k-1 \choose \ell}\\
    %     &= \sum_{\ell = 0}^{n-1} \sum_{k = 0}^{n - \ell - 1} {n-1 \choose k} {i+1 \choose k+1} {n-k-1 \choose \ell}\\
    %     &= \sum_{\ell = 0}^{n-1} \sum_{k=0}^{\ell} {n-1 \choose k} {i+1 \choose k+1} {n-k-1 \choose n-\ell - 1}\\
    %     &= \sum_{\ell = 0}^{n-1} \sum_{k=0}^{\ell} {n-1 \choose n-\ell - 1} {\ell \choose k} {i+1 \choose k+1}\\
    %     &= \sum_{\ell = 0}^{n-1} {n-1 \choose \ell} \sum_{k=0}^{\ell} {\ell \choose k} {i+1 \choose k+1} \\
    %     &= \sum_{\ell = 0}^{n-1} {n-1 \choose \ell} {i+\ell+1 \choose \ell + 1} \\
    %     &= \sum_{\ell = 0}^{n-1} {n-1 \choose \ell} {i+\ell+1 \choose i}
    % \end{align}
\end{proof}


% ------------------------- %
% A 2D recurrence           %
% ------------------------- %
\begin{proposition}
    The characteristic polynomial of $\widetilde{\mathbf{M}}_n$ is
    \begin{equation}
    P_n(z)
    = \sum_{\ell = 0}^{\lfloor \sfrac{n}{2} \rfloor}
    {n \choose 2\ell}
    \bigg(\frac{z}{2} - 1\bigg)^{n - 2\ell}\bigg(1 + \frac{z^2}{4}\bigg)^{\ell} + \dfrac{z}{2}\sum_{\ell = 0}^{\lfloor \frac{n-1}{2}\rfloor}
    {n \choose 2\ell + 1}
    \bigg(\frac{z}{2} - 1\bigg)^{n - 2\ell - 1}\bigg(1 + \frac{z^2}{4}\bigg)^{\ell} \>.
    \end{equation}
\end{proposition}
\begin{proof}
From Proposition~\ref{prop:charpolyrec1_UHT} 
\begin{align}
    P_n(z) &= zP_{n-1}(z) - \sum_{k=1}^n s^{k-1} t_k P_{n-k}(z)\\
    &= zP_{n-1}(z) - \sum_{k=0}^{n-1} s^{n-k+1} t_{n-k} P_k(z)\\
    &= zP_{n-1}(z) - s^{n+1} \sum_{k=0}^{n-1} s^k t_{n-k} P_k(z) \>.
\end{align}

If $s = -1$ and $t_k = 1$ for $1 \le k \le n$,
\begin{equation}
    P_n(z) = zP_{n-1}(z) + (-1)^n\sum_{k=0}^{n-1}(-1)^kP_k(z)
\end{equation}
so
\begin{equation}
    (-1)^nP_n(z) = -z(-1)^{n-1}P_{n-1}(z) + \sum_{k=0}^{n-1}(-1)^kP_k(z) \>.
\end{equation}
Put $Q_k(z) = (-1)^kP_k(z)$. Then
\begin{equation}
    Q_n(z) = -zQ_{n-1}(z) + \sum_{k=0}^{n-1}Q_k(z) \>.
\end{equation}
Put $T_j(z) = \sum_{k=0}^{j} Q_k(z)$. $T_n(z) = T_{n-1}(z) + Q_{n}(z)$, so
\begin{align}
    Q_n(z) &= -zQ_{n-1}(z) + T_{n-1}(z) \\
    T_n(z) &= -zQ_{n-1}(z) + 2T_{n-1}(z)
\end{align}
or
\begin{align}
    \left[
        \begin{array}{c}
            Q_n(z) \\
            T_n(z)
        \end{array}
    \right]
    &=
    \left[
        \begin{array}{cc}
            -z & 1 \\
            -z & 2
        \end{array}
    \right]^n
    \left[
        \begin{array}{c}
            Q_0(z) \\
            s(z)
        \end{array}
    \right] \\
    &= 
    \left[
        \begin{array}{cc}
            -z & 1 \\
            -z & 2
        \end{array}
    \right]^n 
    \left[
        \begin{array}{c}
            1 \\
            1
        \end{array}
    \right]
\end{align}
since $P_0(z) = 1 = (-1)^0Q_0(z)$ and $s(z) = \sum_{j = 0}^0Q_0(z) = 1$. The eigenvalues of this matrix are
\begin{align}
    \lambda_{+} &= 1 - \frac{z}{2} + \Delta \\
    \lambda_{-} &= 1 - \frac{z}{2} - \Delta \\
    \Delta &= \sqrt{1 + \sfrac{z^2}{4}} \>.
\end{align}
If $z = \pm2i$ the eigenvalues are multiple and our formula will have to be modified. The eigenvectors are
\begin{equation}
    \mathbf{V} =
    \left[
        \begin{array}{cc}
            1 & 1 \\
            1 + \frac{z}{2} + \Delta & 1 + \frac{z}{2} - \Delta
        \end{array}
    \right]
\end{equation}
and
\begin{equation}
    \mathbf{V}^{-1} = \dfrac{-1}{2\Delta}
    \left[
        \begin{array}{cc}
            1 + \frac{z}{2} - \Delta & -1 \\
            -1 - \frac{z}{2} - \Delta & 1
        \end{array}
    \right]
\end{equation}
hence
\begin{equation}
    \mathbf{V}^{-1}
    \left[
        \begin{array}{c}
            1 \\
            1
        \end{array}
    \right]
    =
    \dfrac{-1}{2\Delta}
    \left[
        \begin{array}{c}
            \frac{z}{2} - \Delta \\
            \frac{-z}{2} - \Delta
        \end{array}
    \right]
    =
    \left[
        \begin{array}{c}
            \frac{1}{2} - \frac{z}{4\Delta} \\
            \frac{1}{2} + \frac{z}{4\Delta}
        \end{array}
    \right] \>.
\end{equation}
Therefore
\begin{equation}
    \left[
        \begin{array}{c}
            Q_n(z) \\
            T_n(z)
        \end{array}
    \right]
    =
    \left[
        \begin{array}{cc}
            1 & 1 \\
            1 + \frac{z}{2} + \Delta & 1 + \frac{z}{2} - \Delta
        \end{array}
    \right]
    \left[
        \begin{array}{c}
            \lambda_{+}^{n}\left(\frac{1}{2} - \frac{z}{4\Delta}\right) \\
            \lambda_{-}^{n}\left(\frac{1}{2} + \frac{z}{4\Delta}\right)
        \end{array}
    \right]
\end{equation}
and in particular
\begin{equation}
    Q_n(z) = \lambda_{+}^{n}\bigg(\frac{1}{2} - \frac{z}{4\Delta}\bigg) + \lambda_{-}^{n}\bigg(\frac{1}{2} + \frac{z}{4\Delta}\bigg) \>.
\end{equation}
Thus
\begin{align}
    P_n(z) &= \left(-1\right)^{n}Q_n(z) \\
    &= (-\lambda_{+})^{n}\bigg(\frac{1}{2} - \frac{z}{4\Delta}\bigg) + \left(-\lambda_{-}\right)^{n}\bigg(\frac{1}{2} + \frac{z}{4\Delta}\bigg) \>.
\end{align}
Now
\begin{align}
    \left(-\lambda_{+}\right)^{n} &= \bigg(\frac{z}{2} - 1 - \Delta\bigg)^{n} \\
    &= \sum_{k=0}^{n}
    {n \choose k}
    \bigg(
        \frac{z}{2} - 1
    \bigg)^{n-k}
    \left(-\Delta\right)^{k}
\end{align}
and
\begin{align}
    \left(-\lambda_{-}\right)^{n} &= \bigg(\frac{z}{2} - 1 + \Delta\bigg)^n \\
    &= \sum_{k=0}^{n}
    {n \choose k}
    \bigg(\frac{z}{2} - 1\bigg)^{n-k}\Delta^{k} \>.
\end{align}
\begin{multline}
    \therefore P_n(z) = \sum_{k=0}^{n}
    {n \choose k}
    \bigg(\frac{z}{2} - 1\bigg)^{n-k}\bigg(\frac{1}{2}\Delta^{k} + \frac{1}{2}(-\Delta)^{k}\bigg) \\+ \dfrac{z}{4\Delta}\sum_{k=0}^{n}
    {n \choose k}
    \bigg(\frac{z}{2} - 1\bigg)^{n-k}\left(\Delta^{k} - (-\Delta)^{k}\right)\>.
\end{multline}
Every odd term drops out of the first, and every even the second.
\begin{align}
    \therefore P_n(z) &= \sum_{\substack{k = 0 \\ k \text{ even}}}^{n}
    {n \choose k}
    \bigg(\frac{z}{2} - 1\bigg)^{n - k}\Delta^{k} + \dfrac{z}{4\Delta}\sum_{\substack{k = 0 \\ k \text{ odd}}}^{n}
    {n \choose k}
    \bigg(\frac{z}{2} - 1\bigg)^k \cdot2\Delta^k \\
    &= \sum_{\ell = 0}^{\lfloor \sfrac{n}{2} \rfloor}
    {n \choose 2\ell}
    \bigg(\frac{z}{2} - 1\bigg)^{n - 2\ell}\bigg(1 + \frac{z^2}{4}\bigg)^{\ell} + \dfrac{z}{2}\sum_{\ell = 0}^{\lfloor \frac{n-1}{2}\rfloor}
    {n \choose 2\ell + 1}
    \bigg(\frac{z}{2} - 1\bigg)^{n - 2\ell - 1}\bigg(1 + \frac{z^2}{4}\bigg)^{\ell} \>.
\end{align}
At this point the difficulty with $\Delta = 0$ has been resolved by continuity. We see that $P_n(z)$ is a polynomial of degree $n$.
\end{proof}

